Unifying Treatment of Discord via Relative Entropy

A new form of zero-discord state via Petz's monotonicity condition on relative entropy with equality has been derived systematically. A generalization of symmetric zero-discord states is presented and the related physical implications are discussed.

==> preamble.tex <==

%-----------------------------------------------------------------------------%
% Fonts:
%-----------------------------------------------------------------------------%

\usepackage[T1]{fontenc}
\usepackage[sc]{mathpazo}
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{enumerate}
\usepackage{amsthm}% theorems and proofs
\usepackage{amsfonts,mathrsfs}
%-----------------------------------------------------------------------------%
% Margins:
%-----------------------------------------------------------------------------%

\setlength{\topmargin}{0in} \setlength{\headheight}{0in}
\setlength{\headsep}{0.0in} \setlength{\textheight}{8.85in}
\setlength{\oddsidemargin}{0in} \setlength{\evensidemargin}{0in}
\setlength{\textwidth}{6.5in}

%-----------------------------------------------------------------------------%
% PDF:
%-----------------------------------------------------------------------------%

\usepackage{hyperref}
\hypersetup{pdfpagemode=UseNone}

%-----------------------------------------------------------------------------%
% Macros:
%-----------------------------------------------------------------------------%

\newcommand{\comment}[1]{\begin{quote}\sf [*** #1 ***]\end{quote}}
\newcommand{\tinyspace}{\mspace{1mu}}
\newcommand{\microspace}{\mspace{0.5mu}}
\newcommand{\op}[1]{\operatorname{#1}}

\newcommand{\abs}[1]{\left\lvert\tinyspace #1 \tinyspace\right\rvert}
\newcommand{\ceil}[1]{\left\lceil #1 \right\rceil}
\newcommand{\floor}[1]{\left\lfloor #1 \right\rfloor}
\newcommand{\norm}[1]{\left\lVert\tinyspace #1 \tinyspace\right\rVert}
\newcommand{\triplenorm}[1]{
  \left|\!\microspace\left|\!\microspace\left| #1
  \right|\!\microspace\right|\!\microspace\right|}

\renewcommand{\det}{\operatorname{Det}}
\renewcommand{\t}{{\scriptscriptstyle\mathsf{T}}}
\newcommand{\ip}[2]{\left\langle #1 , #2\right\rangle}
\newcommand{\sip}[2]{\langle #1 , #2\rangle}
\newcommand{\fid}{\operatorname{F}}
\newcommand{\setft}[1]{\mathrm{#1}}
\newcommand{\lin}[1]{\setft{L}\left(#1\right)}
\newcommand{\density}[1]{\setft{D}\left(#1\right)}
\newcommand{\unitary}[1]{\setft{U}\left(#1\right)}
\newcommand{\trans}[1]{\setft{T}\left(#1\right)}
\newcommand{\channel}[1]{\setft{C}\left(#1\right)}
\newcommand{\herm}[1]{\setft{Herm}\left(#1\right)}
\newcommand{\pos}[1]{\setft{Pos}\left(#1\right)}
\newcommand{\pd}[1]{\setft{Pd}\left(#1\right)}
\newcommand{\sep}[1]{\setft{Sep}\left(#1\right)}
\newcommand{\sepd}[1]{\setft{SepD}\left(#1\right)}
\newcommand{\ppt}[1]{\setft{PPT}\left(#1\right)}
\newcommand{\sphere}[1]{\setft{S}\left(#1\right)}
\newcommand{\opset}[3]{\setft{#1}_{#2}\left(#3\right)}
\renewcommand{\vec}{\op{vec}}
\newcommand{\im}{\op{im}}
\newcommand{\rank}{\op{rank}}
\newcommand{\spn}{\op{span}}
\newcommand{\sign}{\op{sign}}
\newcommand{\reg}[1]{\mathsf{#1}}

\def\complex{\mathbb{C}}
\def\real{\mathbb{R}}
\def\natural{\mathbb{N}}
\def\integer{\mathbb{Z}}
\def\I{\mathbb{1}}
\def \lket {\left|}
\def \rket {\right\rangle}
\def \lbra {\left\langle}
\def \rbra {\right|}

\newenvironment{mylist}[1]{\begin{list}{}{
    \setlength{\leftmargin}{#1}
    \setlength{\rightmargin}{0mm}
    \setlength{\labelsep}{2mm}
    \setlength{\labelwidth}{8mm}
    \setlength{\itemsep}{0mm}}}
    {\end{list}}

\renewcommand{\baselinestretch}{1.3}


%======================================================================================================================

\def\ot{\otimes}
\def\CP{\mathrm{CP}}
\newcommand{\inner}[2]{\langle #1 , #2\rangle}
\newcommand{\iinner}[2]{\langle #1 | #2\rangle}
\newcommand{\out}[2]{| #1\rangle\langle #2 |}
\newcommand{\Inner}[2]{\left\langle #1 , #2\right\rangle}
\newcommand{\Innerm}[3]{\left\langle #1 \left| #2 \right| #3 \right\rangle}
\newcommand{\defeq}{\stackrel{\smash{\textnormal{\tiny def}}}{=}}
\newcommand{\cls}[1]{\mathrm{#1}}
\newcommand{\Herm}{\mathrm{Herm}}
\newcommand{\OT}[2]{#1 \otimes #2}

%======================================================================================================================

% parentheses, brakets, and sets
\newcommand{\pa}[1]{(#1)}
\newcommand{\Pa}[1]{\left(#1\right)}
\newcommand{\br}[1]{[#1]}
\newcommand{\Br}[1]{\left[#1\right]}
%\newcommand{\br}[1]{\pa{#1}}
%\newcommand{\Br}[1]{\Pa{#1}}
\newcommand{\set}[1]{\{#1\}}
\newcommand{\Set}[1]{\left\{#1\right\}}

%=======================================================================================================================

%Dirac notation
\newcommand{\bra}[1]{\langle#1|}
\newcommand{\Bra}[1]{\left\langle#1\right|}
\newcommand{\ket}[1]{|#1\rangle}
\newcommand{\Ket}[1]{\left|#1\right\rangle}
\newcommand{\braket}[1]{\langle#1\rangle}
\newcommand{\Braket}[1]{\left\langle#1\right\rangle}

%=======================================================================================================================

% the Choi-Jamiolkowski isomorphism
%\DeclareMathOperator{\Jamiolkowski}{J}
\def\Jamiolkowski{J}
\newcommand{\jam}[1]{\Jamiolkowski\pa{#1}}
\newcommand{\Jam}[1]{\Jamiolkowski\Pa{#1}}


%=======================================================================================================================

% the matrix-vector correspondence
%\newcommand{\col}[1]{|#1\rangle}
%\newcommand{\row}[1]{\langle#1|}
%\newcommand{\Col}[1]{\left|#1\right\rangle}
%\newcommand{\Row}[1]{\left\langle#1\right|}
\DeclareMathOperator{\vectorize}{vec}
\newcommand{\col}[1]{\vectorize\pa{#1}}
\newcommand{\row}[1]{\vectorize\pa{#1}^{\dagger}}
\newcommand{\Col}[1]{\vectorize\Pa{#1}}
\newcommand{\Row}[1]{\vectorize\Pa{#1}^{\dagger}}

% the trace of an operator/matrix
\DeclareMathOperator{\trace}{Tr}
\newcommand{\ptr}[2]{\trace_{#1}\pa{#2}}
\newcommand{\Ptr}[2]{\trace_{#1}\Pa{#2}}
\newcommand{\tr}[1]{\ptr{}{#1}}
\newcommand{\Tr}[1]{\Ptr{}{#1}}

%=======================================================================================================================

% Norms
\newcommand{\Abs}[1]{\left|\tinyspace#1\tinyspace\right|}
\newcommand{\Norm}[1]{\left\lVert\tinyspace#1\tinyspace\right\rVert}
\newcommand{\fnorm}[1]{\norm{#1}_{\mathrm{F}}}
\newcommand{\Fnorm}[1]{\Norm{#1}_{\mathrm{F}}}
\newcommand{\tnorm}[1]{\norm{#1}_{\trace}}
\newcommand{\Tnorm}[1]{\Norm{#1}_{\trace}}
\newcommand{\dnorm}[1]{\norm{#1}_{\diamond}}
\newcommand{\Dnorm}[1]{\Norm{#1}_{\diamond}}
\newcommand{\snorm}[2]{\norm{#1}_{\diamond{#2}}}
\newcommand{\Snorm}[2]{\Norm{#1}_{\diamond{#2}}}

%=======================================================================================================================

% Fonts
\newcommand{\fontmapset}{\mathbf} % sets of mappings
\newcommand{\hilb}{\mathcal}      % Hilbert spaces

%=======================================================================================================================

% Sets of operators
\newcommand{\mset}[2]{\fontmapset{#1}\pa{#2}}
\newcommand{\Mset}[2]{\fontmapset{#1}\Pa{#2}}
\newcommand{\Lin}[1]{\Mset{L}{#1}}
\newcommand{\her}[1]{\mset{H}{#1}}
\newcommand{\Her}[1]{\Mset{H}{#1}}
\newcommand{\Pos}[1]{\Mset{H^+}{#1}}
%\newcommand{\tp} [2]{\mset{TP}{#1 \to #2}}
%\newcommand{\TP} [2]{\Mset{TP}{#1 \to #2}}

%=======================================================================================================================

% the Identity super-operator
\newcommand{\identity}{\mathbbm{1}}
%\newcommand{\idsup}[1]{\identity_{\lin{#1}}}
\newcommand{\idsup}[1]{\identity_{#1}}



%=======================================================================================================================
% Hilbert space shortcuts

\def\cA{\mathcal{A}}\def\cB{\mathcal{B}}\def\cC{\mathcal{C}}\def\cD{\mathcal{D}}\def\cE{\mathcal{E}}
\def\cF{\mathcal{F}}\def\cG{\mathcal{G}}\def\cH{\mathcal{H}}\def\cI{\mathcal{I}}\def\cJ{\mathcal{J}}
\def\cK{\mathcal{K}}\def\cL{\mathcal{L}}\def\cM{\mathcal{M}}\def\cN{\mathcal{N}}\def\cO{\mathcal{O}}
\def\cP{\mathcal{P}}\def\cQ{\mathcal{Q}}\def\cR{\mathcal{R}}\def\cS{\mathcal{S}}\def\cT{\mathcal{T}}
\def\cU{\mathcal{U}}\def\cV{\mathcal{V}}\def\cW{\mathcal{W}}\def\cX{\mathcal{X}}\def\cY{\mathcal{Y}}
\def\cZ{\mathcal{Z}}

%=======================================================================================================================

\def\bA{\mathbf{A}}\def\bB{\mathbf{B}}\def\bC{\mathbf{C}}\def\bD{\mathbf{D}}\def\bE{\mathbf{E}}
\def\bF{\mathbf{F}}\def\bG{\mathbf{G}}\def\bH{\mathbf{H}}\def\bI{\mathbf{I}}\def\bJ{\mathbf{J}}
\def\bK{\mathbf{K}}\def\bL{\mathbf{L}}\def\bM{\mathbf{M}}\def\bN{\mathbf{N}}\def\bO{\mathbf{O}}
\def\bP{\mathbf{P}}\def\bQ{\mathbf{Q}}\def\bR{\mathbf{R}}\def\bS{\mathbf{S}}\def\bT{\mathbf{T}}
\def\bU{\mathbf{U}}\def\bV{\mathbf{V}}\def\bW{\mathbf{W}}\def\bX{\mathbf{X}}\def\bY{\mathbf{Y}}
\def\bZ{\mathbf{Z}}

%=======================================================================================================================

\def\rA{\mathrm{A}}\def\rB{\mathrm{B}}\def\rC{\mathrm{C}}\def\rD{\mathrm{D}}\def\rE{\mathrm{E}}
\def\rF{\mathrm{F}}\def\rG{\mathrm{G}}\def\rH{\mathrm{H}}\def\rI{\mathrm{I}}\def\rJ{\mathrm{J}}
\def\rK{\mathrm{K}}\def\rL{\mathrm{L}}\def\rM{\mathrm{M}}\def\rN{\mathrm{N}}\def\rO{\mathrm{O}}
\def\rP{\mathrm{P}}\def\rQ{\mathrm{Q}}\def\rR{\mathrm{R}}\def\rS{\mathrm{S}}\def\rT{\mathrm{T}}
\def\rU{\mathrm{U}}\def\rV{\mathrm{V}}\def\rW{\mathrm{W}}\def\rX{\mathrm{X}}\def\rY{\mathrm{Y}}
\def\rZ{\mathrm{Z}}

%=======================================================================================================================

\def\sA{\mathscr{A}}\def\sB{\mathscr{B}}\def\sC{\mathscr{C}}\def\sD{\mathscr{D}}\def\sE{\mathscr{E}}
\def\sF{\mathscr{F}}\def\sG{\mathscr{G}}\def\sH{\mathscr{H}}\def\sI{\mathscr{I}}\def\sJ{\mathscr{J}}
\def\sK{\mathscr{K}}\def\sL{\mathscr{L}}\def\sM{\mathscr{M}}\def\sN{\mathscr{N}}\def\sO{\mathscr{O}}
\def\sP{\mathscr{P}}\def\sQ{\mathscr{Q}}\def\sR{\mathscr{R}}\def\sS{\mathscr{S}}\def\sT{\mathscr{T}}
\def\sU{\mathscr{U}}\def\sV{\mathscr{V}}\def\sW{\mathscr{W}}\def\sX{\mathscr{X}}\def\sY{\mathscr{Y}}
\def\sZ{\mathscr{Z}}

%=======================================================================================================================

\def\A{\textsf{A}}\def\B{\textsf{B}}\def\C{\textsf{C}}\def\D{\textsf{D}}\def\E{\textsf{E}}
\def\F{\textsf{F}}\def\G{\textsf{G}}\def\H{\textsf{H}}                  \def\J{\textsf{J}}
\def\K{\textsf{K}}\def\L{\textsf{L}}\def\M{\textsf{M}}\def\N{\textsf{N}}\def\O{\textsf{O}}
\def\P{\textsf{P}}\def\Q{\textsf{Q}}\def\R{\textsf{R}}\def\S{\textsf{S}}\def\T{\textsf{T}}
\def\U{\textsf{U}}\def\V{\textsf{V}}\def\W{\textsf{W}}\def\X{\textsf{X}}\def\Y{\textsf{Y}}
\def\Z{\textsf{Z}}

%=======================================================================================================================

\newtheorem{thrm}{Theorem}[section]
\newtheorem{lem}[thrm]{Lemma}
\newtheorem{prop}[thrm]{Proposition}
\newtheorem{cor}[thrm]{Corollary}
\theoremstyle{definition}
\newtheorem{definition}[thrm]{Definition}
\newtheorem{remark}[thrm]{Remark}
\newtheorem{exam}[thrm]{Example}
\numberwithin{equation}{section}

%-----------------------------------------------------------------------------%
% Question environment:
%-----------------------------------------------------------------------------%

\newcounter{questionnumber}
\newenvironment{question}
       {\begin{mylist}{\parindent}
     \item[\stepcounter{questionnumber}\thequestionnumber.]}
       {\end{mylist}}

